Ramsey numbers for partially-ordered sets

We present a refinement of Ramsey numbers by considering graphs with a partial ordering on their vertices. This is a natural extension of the ordered Ramsey numbers. We formalize situations in which we can use arbitrary families of partially-ordered sets to form host graphs for Ramsey problems. We explore connections to well studied Tur\'an-type problems in partially-ordered sets, particularly those in the Boolean lattice. We find a strong difference between Ramsey numbers on the Boolean lattice and ordered Ramsey numbers when the partial ordering on the graphs have large antichains.

==> tables/blank.tex <==
\begin{tabular}[h]{r||c|c|c}& matching2& matching3& matching4\\\hline&&&\\[-2.5ex]\hline
chain2  & 2 & 3 & 3\\\hline
chain3  & 3 & 4 & 4\\\hline
chain4  & 4 &  & \\\hline
chain5  & 5 &  & \\\end{tabular}

==> tables/br.tex <==
\begin{table}[htp]\centering
{\scalebox{0.65}{
\begin{tabular}[h]{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|l|}
\hline
 & \multicolumn{1}{l@{\hspace{-1.3mm}}}{\rot{b2}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cap2}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cap3}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cap4}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cap5}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cap6}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{chain2}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{chain3}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{chain4}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{chain5}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{crown2}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{crown3}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{crown4}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{crown5}} & \multicolumn{1}{l@{\hspace{-4.0mm}}}{\rot{crown6}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cup2}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cup3}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cup4}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cup5}} & \multicolumn{1}{l@{\hspace{-2.7mm}}}{\rot{cup6}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{diamond2}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{diamond3}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{diamond4}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{diamond5}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{diamond6}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{matching2}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{matching3}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{matching4}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{matching5}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{matching6}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{standard3}} & \multicolumn{1}{l@{\hspace{-6.0mm}}}{\rot{standard4}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark1l1}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark1l2}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark1l3}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark1l4}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark2l1}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark2l2}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark2l3}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark3l1}} & \multicolumn{1}{l@{\hspace{-5.3mm}}}{\rot{stark3l2}} & \multicolumn{1}{l|}{\rot{stark4l1}} \\\hline\\[-2.5ex]\hline
b2  &  & 4  & 4  &  &  &  & 2  & 4  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 3  & 4  & 4  & 4  &  &  &  & 4  &  &  &  &  &  &  &  &  & \\\hline
cap2  & 4  & 2  & 3  & 3  & 3  & 3  & 2  & 3  & 4  & 5  & 4  & 4  & 4  & 4  & 4  & 3  & 3  & 4  & 4  & 4  & 4  & 4  & 4  & 4  &  & 3  & 3  & 4  & 4  & 4  & 4  & 4  & 3  & 4  & 4  &  & 3  & 4  & 4  & 4  &  & 4 \\\hline
cap3  & 4  & 3  & 3  & 3  & 3  & 4  &  & 3  & 4  &  & 4  & 4  & 4  & 4  &  & 3  & 4  & 4  &  &  & 4  &  &  &  &  & 3  & 4  & 4  & 4  & 4  & 4  &  & 3  & 4  &  &  & 4  &  &  & 4  &  & 4 \\\hline
cap4  &  & 3  & 3  & 3  & 4  & 4  &  & 4  &  &  & 4  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  & 4  &  &  &  & 4  &  &  & 4  &  & 4 \\\hline
cap5  &  & 3  & 3  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
cap6  &  & 3  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
chain2  & 2  & 2  &  &  &  &  &  &  &  &  & 3  &  &  &  &  & 2  &  &  &  &  & 2  &  &  &  &  & 2  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
chain3  & 4  & 3  & 3  & 4  &  &  &  & 4  &  &  & 4  &  &  &  &  & 3  & 3  & 4  &  &  & 4  &  &  &  &  & 3  & 4  & 4  & 4  & 4  &  &  & 4  & 5  & 5  &  & 5  &  &  & 5  &  & \\\hline
chain4  &  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 4  & 5  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
chain5  &  & 5  &  &  &  &  &  &  &  &  &  &  &  &  &  & 5  &  &  &  &  &  &  &  &  &  & 5  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
crown2  &  & 4  & 4  & 4  &  &  & 3  & 4  &  &  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  & 3  & 4  & 4  & 4  & 4  &  &  & 4  &  &  &  &  &  &  &  &  & \\\hline
crown3  &  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 3  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
crown4  &  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
crown5  &  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
crown6  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
cup2  & 4  & 3  & 3  & 4  & 4  & 4  & 2  & 3  & 4  & 5  & 4  & 4  & 4  & 4  & 4  & 2  & 3  & 3  & 3  & 3  & 4  & 4  & 4  & 4  &  & 3  & 3  & 4  & 4  & 4  & 4  & 4  & 3  & 3  & 4  & 4  & 4  & 4  &  & 4  & 4  & \\\hline
cup3  & 4  & 3  & 4  & 4  &  &  &  & 3  & 4  &  & 4  & 4  & 4  & 4  &  & 3  & 3  & 3  & 3  & 4  & 4  &  &  &  &  & 3  & 4  & 4  & 4  & 4  & 4  &  & 3  & 4  & 4  & 4  & 4  &  &  &  &  & \\\hline
cup4  &  & 4  & 4  &  &  &  &  & 4  &  &  & 4  &  &  &  &  & 3  & 3  & 3  & 4  & 4  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  & 4  & 4  & 4  & 4  &  &  &  &  &  & \\\hline
cup5  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 3  & 3  & 4  & 4  & 4  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
cup6  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 3  & 4  & 4  & 4  & 4  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
diamond2  &  & 4  & 4  &  &  &  & 2  & 4  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 3  & 4  & 4  & 4  &  &  &  & 4  &  &  &  &  &  &  &  &  & \\\hline
diamond3  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
diamond4  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
diamond5  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
diamond6  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
matching2  & 3  & 3  & 3  & 4  & 4  & 4  & 2  & 3  & 4  & 5  & 3  & 3  & 4  & 4  & 4  & 3  & 3  & 4  & 4  & 4  & 3  & 4  & 4  & 4  & 4  & 3  & 3  & 4  & 4  & 4  & 3  & 4  & 3  & 4  & 4  &  & 4  & 4  &  & 4  &  & \\\hline
matching3  & 4  & 3  & 4  & 4  & 4  & 4  &  & 4  & 5  &  & 4  & 4  & 4  & 4  & 4  & 3  & 4  & 4  & 4  & 4  & 4  &  &  &  &  & 3  & 3  & 4  & 4  & 4  & 4  & 4  & 4  & 4  &  &  & 4  & 4  &  &  &  & \\\hline
matching4  & 4  & 4  & 4  & 4  & 4  & 4  &  & 4  &  &  & 4  & 4  & 4  & 4  & 4  & 4  & 4  & 4  & 4  & 4  & 4  &  &  &  &  & 4  & 4  & 4  & 4  & 4  & 4  &  & 4  & 4  &  &  & 4  & 4  &  &  &  & \\\hline
matching5  & 4  & 4  & 4  & 4  & 4  &  &  & 4  &  &  & 4  & 4  & 4  & 4  &  & 4  & 4  & 4  & 4  &  & 4  &  &  &  &  & 4  & 4  & 4  & 4  & 4  & 4  &  & 4  & 4  &  &  & 4  &  &  &  &  & \\\hline
matching6  &  & 4  & 4  &  &  &  &  & 4  &  &  & 4  & 4  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  & 4  &  & 4  &  &  &  &  &  &  &  &  & \\\hline
standard3  &  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 3  & 4  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
standard4  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
stark1l1  & 4  & 3  & 3  & 4  &  &  &  & 4  &  &  & 4  &  &  &  &  & 3  & 3  & 4  &  &  & 4  &  &  &  &  & 3  & 4  & 4  & 4  & 4  &  &  & 4  & 5  & 5  &  & 5  &  &  & 5  &  & \\\hline
stark1l2  &  & 4  & 4  &  &  &  &  & 5  &  &  &  &  &  &  &  & 3  & 4  & 4  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  & 5  & 5  &  &  &  &  &  &  &  & \\\hline
stark1l3  &  & 4  &  &  &  &  &  & 5  &  &  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  & 5  &  &  &  &  &  &  &  &  & \\\hline
stark1l4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
stark2l1  &  & 3  & 4  & 4  &  &  &  & 5  &  &  &  &  &  &  &  & 4  & 4  &  &  &  &  &  &  &  &  & 4  & 4  & 4  & 4  &  &  &  & 5  &  &  &  & 5  &  &  &  &  & \\\hline
stark2l2  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
stark2l3  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
stark3l1  &  & 4  & 4  & 4  &  &  &  & 5  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  & 5  &  &  &  &  &  &  &  &  & \\\hline
stark3l2  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
stark4l1  &  & 4  & 4  & 4  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\\hline
\end{tabular}}}

\vspace{1em}
\caption{\label{tab:br}Computed Boolean Ramsey Numbers}
\end{table}

